Momentum Q-learning with Finite-Sample Convergence Guarantee

Existing studies indicate that momentum ideas in conventional optimization can be used to improve the performance of Q-learning algorithms. However, the finite-sample analysis for momentum-based Q-learning algorithms is only available for the tabular case without function approximations. This paper analyzes a class of momentum-based Q-learning algorithms with finite-sample guarantee. Specifically, we propose the MomentumQ algorithm, which integrates the Nesterov's and Polyak's momentum schemes, and generalizes the existing momentum-based Q-learning algorithms. For the infinite state-action space case, we establish the convergence guarantee for MomentumQ with linear function approximations and Markovian sampling. In particular, we characterize the finite-sample convergence rate which is provably faster than the vanilla Q-learning. This is the first finite-sample analysis for momentum-based Q-learning algorithms with function approximations. For the tabular case under synchronous sampling, we also obtain a finite-sample convergence rate that is slightly better than the SpeedyQ \citep{azar2011speedy} when choosing a special family of step sizes. Finally, we demonstrate through various experiments that the proposed MomentumQ outperforms other momentum-based Q-learning algorithms.

==> plan.tex <==
JMLR plan (before Mid Feb. 2020)
1> We should acknowledge the NeSA work. Pointing out the different emphasis of the two work. The reviewer's work is focused on asymptotic analysis, no finite time bound. Our work focus on the finite time bound.
1.1> emphasize the hyper paramter m, strictly better PAC bound than Speedy Q.
1.2> Prove stability of the iteration
1.3> Prove the asynchronous sampling case
1.4> Re-organize the proof

2> Experiment of PAQL and finish the writeup of the experiment section for JMLR submission.
3> Add results for linear function approximation: exponential rate and advantage over vanilla Q-learning.


 
CDC plan (Due Mar 17th, 2020)
1> Similar to <1> "JMLR plan"
2> Proof and Experiment for Async Tabular version
3> Remove experiments of parametric Q-learning
